Economic Efficiency Requires Interaction

We study the necessity of interaction between individuals for obtaining approximately efficient allocations. The role of interaction in markets has received significant attention in economic thinking, e.g. in Hayek's 1945 classic paper. We consider this problem in the framework of simultaneous communication complexity. We analyze the amount of simultaneous communication required for achieving an approximately efficient allocation. In particular, we consider two settings: combinatorial auctions with unit demand bidders (bipartite matching) and combinatorial auctions with subadditive bidders. For both settings we first show that non-interactive systems have enormous communication costs relative to interactive ones. On the other hand, we show that limited interaction enables us to find approximately efficient allocations.

==> app/matching-alg-app.tex <==
% !TEX root = ..//communism.tex

%\section{Proofs from Section \ref{sec-matching-alg}}

%\prevproof{Theorem}{thm-auction-alg}{
%Fix some optimal solution $(o_1,...,o_n)$ (every player receives at most one item). Let $N'$, $|N'|=n'$, be the set of players that receive an item in the optimal solution. 
%\begin{definition}
%A player is called \emph{satisfied} if he is either allocated an item or $D_i=\emptyset$.
%\end{definition}
%
%Let $END$ be the random variable that denotes the number of rounds until the first time that $(1-\delta)n'$ players in $N'$ are satisfied. We will prove the following lemma:
%
%\begin{lemma}
%$E[END]\leq \frac {4\log n} {\delta^2}$.
%\end{lemma}
%\begin{proof}
%%helpful?
%The heart of the proof is the definition of two budgets: one for demand halving actions for players in $N'$ and one for price increments. We show that in expectation after at most $\frac {4\log n} {\delta^2}$ rounds at least one of these budgets is exhausted and hence the number of unsatisfied players in $N'$ is at most $\delta n'$. 
% 
%Consider the demand set $D_i$ of some player $i$ at some round $r$. Observe that all items in $D_i$ has the same price $p_{D_i}$. Let $D^{p}_i=S_i\cap \{ j|p_j=p \}$.
%We will use the following claim:
%\begin{claim}
%Consider some round $r$ and suppose that at least $t$ players are unsatisfied in the beginning of that round. Then, either the expected increase in $\Sigma_j p_j$ is at least $t \cdot \frac {\delta} {4}$ or for at least half of the unsatisfied players it holds that $D^{p_{D_i}}_i$ has shrunk by at least a factor of $2$.
%\end{claim}
%\begin{proof}
%Consider some player $i$ that is not satisfied. When it is $i$'s turn to be considered in Step \ref{step-order} either at least half the items in $D_i$ were taken by previous players in the order or not. If at least half the items in $D_i$ were taken by previous players then $D^{p_{D_i}}_i$ has shrunk by a factor of at least $2$. Otherwise, since player $i$ selects $j_i$ at random from $D_i$, with probability of at least $\frac 1 2$ we have that $j_i$ was not taken by any previous player. In this case $i$ the price of $p_{j_i}$ is increased by $\delta$ so the expected increase of some item due to $i$ is $\frac \delta 2$. This implies that either for at least $t/2$ players $D^{p_{D_i}}_i$ has shrunk by at least a factor of $2$ or at least $t/2$ players caused an expected increase of $\delta/2$ in the price of some item. The later implies by linearity of expectation an expected total increase of $t \cdot \frac {\delta} {4}$.
%\end{proof}
%
%Now, notice that the price of each item can be increased at most $\frac 1 \delta$ times (the price increases in increments of $\delta$ and no player demands an item which has a value of $1$). Since an item that was allocated stays allocated and at most $n'$ items can be allocated, we have that the maximal number of increments that the algorithm can make is $\frac {n'} \delta$.
%
%
%In addition, there are $n$ items and the price of an item can only increase, each $D^p_i$ can be shrunk by a factor of $2$ at most $\log n$ time. As previously argued, $p$ can get only $\frac 1 \delta$ different values. The total number of shrinkage steps with respect to players in $N'$ is therefore $\frac {n'\log n} \delta$.
%
%To complete the proof recall that at every round prior to $END$ at least $\delta n'$ players in $N'$ are unsatisfied. By the claim in each round either the expected number of increments is $\frac {\delta n'} 4$ or the expected number of shrinkage steps with respect to players in $N'$ is $\frac {\delta n'}{2}$. In any case, after $\frac {4\log n}{\delta^2}$ rounds we expect that there are no more increments or shrinkage steps with respect to players in $N'$ to make.\end{proof}
%
%\begin{lemma}
%If at least $(1-\delta)n'$ of the players in $N'$ are satisfied then the approximation of the algorithm is $1-2\delta$.
%\end{lemma}
%\begin{proof}
%We use a variant of the first welfare theorem to prove the lemma. Consider a player $i$ that has received an item $j_i$. The player receives an item that maximizes his demand (up to $\delta$), and thus the profit from $j_i$ is at least the profit from the item $o_i$ he got in the optimal solution (up to $\delta$, we allow $o_i=\emptyset$). We therefore have: $v_i(j_i)-p_{j_i}\geq v_i(o_i)-p_{o_i}-\delta$. For each satisfied player $i$ that did not receive any items we have that $0\geq v_i(o_i)-p_{o_i}$. Denote by $N_s$ the set of satisfied players. Summing over all satisfied players we get:
%
%\begin{align*}
%\sum_{i \in N_s}(v_i(j_i)-p_{j_i}) &\geq \sum_{\text{$i\in N_s$ is allocated}}(v_i(o_i)-p_{o_i} -\delta) ~~+\sum_{\text{$i\in N_s$ is unallocated}}(v_i(o_i)-p_{o_i})\\
%&= \sum_{i \in N_s} (v_i(o_i)-p_{o_i}) - \delta n' \\
%ALG - \sum_{j\in N}p_j &\geq OPT - \delta n' - \sum_{i\in N_s}p_{o_i} - n'\delta\\
%ALG &\geq OPT - 2n'\delta = (1-2\delta)n'
%\end{align*}
%where in the third transition we used the facts that items that are unallocated by the algorithm have a price of $0$ and that $N' \cap N_s \geq (1-\delta)N'$.
%\end{proof}}

%\subsection{A $k$-Round Algorithm for Matching}\label{subsec-k-round-matching}
%
%Fix some optimal solution $(o_1,...,o_n)$ (every player receives at most one item). Let $N'$ be the set of players that receive a nonempty bundle in the optimal solution. The following algorithm achieves an approximation ratio of $O(n^{\frac 1 {k+1}})$ in $k$ rounds.
%
%\subsubsection*{The Algorithm}
%\begin{enumerate}
%\item Let $N_1=V_1$ and $U_1=V_2$.
%\item In every round $r=1,\ldots,k$:
%\begin{enumerate}
%\item Each player $i$ selects uniformly at random an item $j_i\in U_i$ that he demands.
%\item\label{step-order-k} Go over the players in $N_r$ in a fixed arbitrary order. Player $i$ receives $j_i$ if this item was not allocated yet.
%\item Let $N_{r+1} \subseteq N_r$ be the set of players that were not allocated items at round $r$ or before.
%\item Let $U_{r+1} \subseteq U_r$ be the set of items that were not allocated at round $r$ or before.
%\end{enumerate}
%\end{enumerate}
%
%\begin{theorem}
%For every $k\leq \log n$, the approximation ratio of the algorithm is $O(n^{\frac 1 {k+1}})$. In particular, when $k=1$ the approximation ratio is $O(\sqrt n)$ and when $k=O(\log n)$ the approximation ratio is $O(1)$.
%\end{theorem}
%
%Consider a run of the algorithm. Let $D_{r,i}\subseteq U_r$ be the set of items that player $i$ demands and are still available immediately before round $r$ starts. Let $X_{r,i}$ be the set of items that where allocated to other players before $i$'s turn in step (\ref{step-order-k}). Player $i$ is said to be \emph{easy to satisfy} if in some round $r$ we have that $D_{r,i}- X_{r,i}\geq \frac {D_{r,i}} {n^{\frac 1 {k+1}}}$. Let $S$ be the event that at least half of the players in $N'$ are easy to satisfy. We will show that $E[ALG|S]=O(\frac {OPT} {n^{\frac 1 {k+1}}})$ and that $E[ALG|\bar S]=O(\frac {OPT} {n^{\frac 1 {k+1}}})$, where $ALG$ is the random variable that denotes the value of the solution that the algorithm outputs. Together this implies that $E[ALG]=O(\frac {OPT} {n^{\frac 1 {k+1}}})$. Each one of the next two lemmas handles one of those cases.
%
%
%\begin{lemma}
%$E[ALG|S]=O(\frac {OPT} {n^{\frac 1 {k+1}}})$.
%\end{lemma}
%\begin{proof}
%Let $C_{i,r}$ be the random variable that denotes the probability that player $i$ is allocated an item at round $r$. Observe that if player $i$ is easy to satisfy then for some round $r$ we have that $E[C_{i,r}]\geq \frac {1} {n^{\frac 1 {k+1}}}$. Let $P$ denote the set of easy to satisfy players. The expected number of easy to satisfy players that are allocated an item is at least $E[\Sigma_{i\in P} C_{i,r}]=\Sigma_{i\in P} E[C_{i,r}]\geq |P|\cdot \frac {1} {n^{\frac 1 {k+1}}} \geq \frac {n'} 2 \cdot \frac {1} {n^{\frac 1 {k+1}}}$. The required approximation ratio follows since the value of the optimal solution is $n'$.
%\end{proof}
%
%\begin{lemma}
%$E[ALG|\bar S]=O(\frac {OPT} {n^{\frac 1 {k+1}}})$.
%\end{lemma}
%\begin{proof}
%Consider a player $i$ that is not easy to satisfy. Observe the for every such player $i$ and round $r$, if $i \in N_r \cap N_{r+1}$ then $|D_{r,i}| \geq n^{\frac{1}{k+1}}| D_{r+1,i}|$. This is true since if such player $i$ was not allocated any items at round $r$ then the set of available items that he demands shrinks. Therefore, for every player $i$ that was not allocated anything at round $k$, we have that $|D_{k+1,i}| \leq n^{\frac{1}{k+1}}$. If there exists a player $i$ such that $|D_{k+1,i}| >0$ then it has to be the case that initially $|D_{1,i}|\geq n^{\frac k {k+1}}$. This implies that at least $n^{\frac k {k+1}}-n^{\frac{1}{k+1}}$ of the items were allocated and hence the approximation ratio is $O(n^{\frac 1 {k+1}})$ (there are $m$ items, so the value of the optimal solution is at most $m$). In any other case for every such player $i$ that was not allocated any bundle we have that $D_{k+1,i}=\emptyset$. In particular, the item $o_i$ that he receives in the optimal solution was allocated. Since there are at least $\frac {n'} 2$ such players, this implies that at least $\frac {n'} 2$ items were allocated and proves the claimed approximation bound in this case as well. 
%\end{proof}

==> app/matching-app.tex <==
% !TEX root = ..//communism.tex

%\section{Proofs from Section \ref{sec-matching-lb}} \label{sec-app-matching-lb}

%\prevproof{Proposition}{prop-matching-trivial} {
%
%The randomized algorithm will be a corollary of the $k$-round algorithm of Subsection \ref{subsec-k-round-matching} ($k=1$). We now describe the deterministic algorithm.
%
%Let $l'=\frac l{\log n}$. We consider the algorithm where each player reports the indices of some arbitrary $l'$ vertices in his neighbor set. The algorithm matches as many reported vertices as possible.
%
%We now analyze the approximation ratio of the algorithm. Consider some optimal matching. We distinguish between two cases. The first one is when at least half of the players that are matched in the optimal solution have at most $l'$ neighbors (call this set $S$). In this case, vertices in $S$ can report their full neighbor set. The algorithm will consider in particular the matching that matches vertices in $S$ as in the optimal solution, and thus we will get a $2$ approximation.
%
%In the second case, most of the players that are matched in the optimal solution have more than $l'$ neighbors (call this set $T$). Consider the matching that the algorithm outputs. If all vertices in $T$ are matched, then we get a $2$ approximation. Otherwise, there is a player $i\in T$ that is not matched by the algorithm. This implies that all the $l'$ vertices that he reported are already matched, and this is a lower bound to the number of matches that the algorithm outputs. The theorem follows since the optimal matching makes at most $n$ matches.
%}

%\subsection{Hardness of Deterministic Matching}\label{subsec-matching-hardness}
%
%In the proof we assume that our graphs are $w$-uniform graphs. That is, the size of neighbor set $\nseti{i}$ for every player $i$ is $w$. Notice that this assumption only makes our hardness result stronger. For this proof, we fix a specific simultaneous algorithm and analyze its properties. 
%
%We begin by considering a specific random construction of graphs that we name $w$-random. In a $w$-random graph we choose $|U|=w$ vertices from $V_2$ uniformly at random and let the neighbor set of each one of the players be $\nseti{i}=U$. Let $(a_1,\ldots,a_n)$ be the output of the algorithm on this instance. As the optimal matching includes exactly $w$ matched players it is clear that the solution outputted by the algorithm matches at most $w$ players. The crux of the proof is constructing a ``fooling instance'', where all players send the same messages and hence the algorithm cannot distinguish the fooling instance from the original instance and outputs the same allocation. We will construct this fooling instance so that on one hand for almost every player $i$, $a_i$ is not in the neighbour set of player $i$ (this will be true to approximately $n-2w$ players). This implies that the value of the matching that the algorithm outputs in the fooling instance is low. On the other hand, the size of the optimal matching in the fooling instance will be $\alpha=\Theta(n)$. 
%
%%The proof of Theorem \ref{thm-matching} is given in Subsection \ref{subsec-matching-hardness}. 
%
%Let $g_i(V)$ denote the message that player $i$ sends when his neighbor set is $V$. Let $G_i(m) = \{V|g_i(V)=m\}$ and $G_i(V)=G_i(g_i(V))$. The main challenge in the proof is constructing a fooling set with a large optimal matching. The next definition provides us the machinery required for proving this:
%
%\begin{definition}
%For a player $i$ and neighbor set $\nseti{i}$, $\nseti{i}$ is \emph{$\alpha$-unsafe} for a vertex $k\notin \nseti{i}$ if $|\cup_{U\in G_i(\nseti{i}), k \notin U} U |\geq \alpha$. Otherwise, we say that $S_i$ is $\alpha$-safe for $k$.
%\end{definition}
%
%For a $w$-random graph we say that player $i$ is $\alpha$-adaptable if the neighbor set $S_i$ is $\alpha$-unsafe for $a_i$. We will first formalize the discussion above by constructing a fooling instance given that there are $|P|$ $\alpha$-adaptable players. Later, we will show that there exists an instance in which $|P|\approx n-2w$ players are $\alpha$-adaptable.
%
%\begin{lemma}
%Consider a $w$-random graph in which a set $P$ of the players are $\alpha$-adaptable. Then, there exists a fooling instance for which at least $\min(|P|,\alpha)$ vertices can be matched, but the algorithm returns a solution with at most $w$ matched vertices.
%\end{lemma}
%\begin{proof}
%The fooling instance is constructed as follows: for each player $i\in P$, let $\nseti{i}'$ be some neighbor set such that $a_i\notin \nseti{i}'$ and $\nseti{i}'\in G_i(\nseti{i})$. Such $\nseti{i}'$ exists since by assumption player $i$ is an $\alpha$-adaptable player which implies that $a_i$ is $\alpha$-unsafe for $\nseti{i}$. For any such choice of $\nseti{i}'$ we have that players in $P$ are still not matched by the algorithm. The number of matchings in the fooling instance is therefore at most $w$. Notice that this argument holds for \emph{any} set of $\nseti{i}'$'s chosen as above.
%
%To guarantee that at least $\min(|P|,\alpha)$ vertices can be matched in the new instance, we have to be more careful in our choice of the $\nseti{i}'$'s. We say that player $i$ with neighbor set $\nseti{i}$ is \emph{interested in} vertex $j\in V_2$ if there exists a neighbor set $\nseti{i}'$ where $a_i\notin \nseti{i}'$, $\nseti{i}' \in G_i(\nseti{i})$, and $j\in \nseti{i}'$. Since for every $i\in P$ we know that $a_i$ is $\alpha$-unsafe for $\nseti{i}$, there exists at least $\alpha$ vertices which player $i$ is interested in. Thus by Hall's marriage theorem there exists a matching of at least $\alpha$ vertices among the players in $P$ where each player is matched to a vertex that he is interested in. This implies that there exists a set of neighbor set $\nseti{i}'$ as above where at least $\min(|P|,\alpha)$ vertices can be matched in the fooling instance.
%\end{proof}
%
%We now show that there exists a $w$-random graph in which the number of $\alpha$-adaptable players is large:
%
%\begin{lemma}\label{lemma-matching-adaptable}
%Let $p=\dfrac{2^l\cdot n{\alpha \choose w}}{{n \choose w} }$. There exists a $w$-random graph in which at least $(1-p)\cdot n-w$ of the players are $\alpha$-adaptable.
%\end{lemma}
%\begin{proof}
%We first show that for each player $i$ the number of neighbor sets that are $\alpha$-safe for at least one vertex is small. 
%\begin{claim}\label{clm-matching-random-v}
%For each player $i$ there are at most $2^l \cdot n{\alpha \choose w}$ possible neighbor sets (of size $w$) that are $\alpha$-safe for at least one vertex. 
%\end{claim}
%\begin{proof}
%Consider a message $m$ and a vertex $k\in V_2$. Observe that by definition for every set $S$ which is $\alpha$-safe for $k$ we have that $S \subseteq \cup_{U\in G_i(\nseti{i}), k \notin U} U$ and that $|\cup_{U\in G_i(\nseti{i}), k \notin U} U|\leq \alpha$. This immediately implies that there are at most ${\alpha \choose w}$ neighbor sets in $G_i(m)$ that are $\alpha$-safe for $k$. This is true for each of the $n$ vertices in $V_2$ and hence there are at most $n{\alpha \choose w}$ neighbor sets in $G_i(m)$ that are $\alpha$-safe for at least one vertex. The proof is completed by observing that there are at most $2^l$ different messages.
%\end{proof}
%
%We are now ready to show that there exists a $w$-random graph with the required number of $\alpha$-adaptable players. Observe that in a $w$-random graph, for each player $i$ the probability that $\nseti{i}$ is $\alpha$-safe for some vertex $k \notin \nseti{i}$ is at most $\dfrac{2^l\cdot n{\alpha \choose w}}{{n \choose w} } =p$. This is simply because by construction the neighbor set $\nseti{i}$ of player $i$ is chosen uniformly at random from all possible neighbor sets (the neighbor sets of any two players are indeed correlated). 
%
%We now show that there exists a $w$-random graph in which there is a set $P'$, $|P'|\geq (1-p) \cdot n$ where for each $i\in P'$ we have that $\nseti{i}$ is $\alpha$-unsafe for every $k \notin \nseti{i}$. To see why this is the case, for each player $i$, let $n_i$ be a random variable that gets a value of $1$ if $\nseti{i}$ is $\alpha$-unsafe for every $k \notin \nseti{i}$ and a value of $0$ otherwise. Let $n'=\Sigma_i n_i$. By the first part, for any player $i$, $E[n_{i}]\geq 1-p$. Using linearity of expectation, $E[n']\geq n\cdot (1-p)$. The claim follows since there must be at least one instance $I$ where $n'\geq E[n']$.
%
%To conclude the proof, observe that in the instance $I$ any player $i\in P$ for which $a_i \notin S_i$ is an $\alpha$-adaptable player. Since there are at most $w$ players for which $a_i \in S_i$ we have that at least $|P'|-w= (1-p)\cdot n-w$ players are $\alpha$-adaptable, as required.
%\end{proof}
%
%Finally, we compute the values of our parameters and show that the theorem indeed holds.
%
%\begin{lemma}
%For $\alpha =\frac{n}{4}$ and $w=2l + \log(n)$, the approximation ratio of a simultaneous algorithm in which each message length is at most $l$ bits is $\dfrac{n}{8l+ 4\log(n)}$.
%\end{lemma}
%\begin{proof}
%We first compute a lower bound on the number of $\alpha$-adaptable players. By Lemma \ref{lemma-matching-adaptable}, we have that the number of $\alpha$-adaptable players is a least $(1-p) \cdot n -w$. By Claim \ref{matching-claim-bound1} below we have that $(1-p)\geq (1-\left( \frac{1}{4} \right)^l)$, thus $(1-p) \cdot n -w>\alpha$. Therefore the approximation ratio of the algorithm is at most $\dfrac{\alpha}{w} = \dfrac{\frac{n}{4}}{2l+ \log(n)} = \dfrac{n}{8l+ 4\log(n)}  $.
%\end{proof}
%
%\begin{claim}\label{matching-claim-bound1}
%For $\alpha =\frac{n}{4}$ and $w=2l + \log(n)$: $p\leq\frac {2^l \cdot n{\alpha \choose w}} {{n \choose w}}  \leq \left( \frac{1}{4} \right)^{ l}$.
%\end{claim}
%\begin{proof}
% \begin{align*}
%\frac {2^l \cdot n{\alpha \choose w}} {{n \choose w}} = 2^l n \cdot \frac{\alpha! \cdot (n-w)!}{(\alpha-w)! \cdot n!}= 2^l n \cdot \frac{\prod_{i=1}^w (\alpha -w+i) }{\prod_{i=1}^w (n -w+i)} \leq 2^l n \cdot \left( \frac{\alpha}{n} \right)^w.
%\end{align*}
%By plugging in the values of $\alpha$ and $w$ we get:
%\begin{align*}
% 2^l n \cdot \left( \frac{\alpha}{n} \right)^w \leq  2^{l} n \cdot \left( \frac{1}{4} \right)^{2l+\log(n)} \leq n \left( \frac{1}{4} \right)^{l+ \log(n)} \leq \left( \frac{1}{4} \right)^{ l}.
%\end{align*}
% \end{proof}


==> app/xos-alg-app.tex <==
% !TEX root = ..//communism.tex

\section{Proofs from Section \ref{sec-xos-alg}}

%\prevproof{Proposition}{prop-restricted-instances}
%{
%The proposition follows from the following three lemmas.
%
%\begin{lemma}
%If there exists a simultaneous algorithm for XOS bidders that provides an approximation ratio of $\alpha$ where each bidder sends a message of length $l$, then there exists a simultaneous algorithm for subadditive bidders that provides an approximation ratio of $O(\alpha\cdot \log m)$ where each bidder sends a message of length $l$.
%\end{lemma}
%\begin{proof}
%For every subadditive valuation there is an XOS valuation that is an $O(\log m)$ approximation of it \cite{D07}\footnote{A valuation $v$ $\alpha$-approximates  a valuation $u$ if for every $S$ we have that $u(S)\geq v(S)\geq \frac{u(S)} \alpha$.}; thus, if each player computes this XOS valuation and proceeds as in the algorithm for XOS valuations we get an algorithm for subadditive valuations, losing only an $O(\log m)$ factor in the approximation ratio.
%\end{proof}
%
%
%\begin{lemma}
%If there exists a simultaneous algorithm for binary XOS bidders (all with the same $\mu$) that provides an approximation ratio of $\alpha$ where each bidder sends a message of length $l$, then there exists a simultaneous algorithm for XOS bidders that provides an approximation ratio of $O(\alpha\cdot \log m)$ where each bidder sends a message of length $O(l \cdot \log m)$.
%\end{lemma}
%\begin{proof}
%We will move from general XOS valuations to binary XOS valuations using the following notion of projections:
%\begin{definition}
%A \emph{$\mu$-projection} of an additive valuation $a'$ is the following additive valuation $a$:
%\begin{eqnarray*}
%a(\{j\})=\left\{
%  \begin{array}{ll}
%    \mu, & \hbox{if $2\mu>a'(j)\geq \mu$;} \\
%    0, & \hbox{otherwise.}
%  \end{array}
%\right.
%\end{eqnarray*}
%\end{definition}
%A \emph{$\mu$-projection} of an XOS valuation $v$ is the XOS valuation $v^\mu$ that consists exactly of all $\mu$-projections of the additive valuations (clauses) that define $v$.
%
%Let $v_{max}$ be $\max_i v_i(M)$ rounded down to the nearest power of $2$. Let $\mathcal M=\{ \frac {v_{max}} {2m}, \frac {v_{max}} {m}, \ldots, \frac {v_{max}} 2, v_{max}\}$. The next claim shows that there exists some $\mu\in \mathcal M$ such that the value of the optimal solution with respect to the $\mu$-projections $v_i^\mu$ is only a logarithmic factor away from the value of the optimal solution with respect to the $v_i$'s. Given the claim below and an algorithm $A$ for binary XOS valuations we can construct the following algorithm for general XOS valuations: each player $i$ computes, for every $\mu\in \{ \frac {MAX_i} {2m}, \frac {MAX_i} {m},  \ldots, \frac {MAX_i} 2, MAX_i\}$, where $MAX_i$ equals $v_i(M)$ rounded down to the nearest power of $2$, his $\mu$-projection and sends both $\mu$ and the message of length $l$ he would have sent in the algorithm $A$ if his valuation was $v_i^\mu$. The new algorithm computes now up to $|\mathcal M|$ different allocations by running $A$ once for each $\mu\in \mathcal M$, and outputs the allocation with the best value\footnote{Observe that if player $i$ does not report a valuation for some value of $\mu \in \mathcal M$ then the algorithm may assume its valuation for this $\mu$ is $0$ for every bundle.}. By the claim below, the approximation ratio is $O(\alpha \cdot \log m)$. The length of the message that each bidder sends is $O(l\cdot \log m)$.
%
%\begin{claim}
%Let $OPT$ be the value of the optimal solution with respect to the $v_i$'s. For every $\mu\in \mathcal M$, let $OPT_\mu$ be the value of the optimal solution with respect to the $\mu$-projections $v_i^\mu$. There exists some $\mu \in \mathcal M$ such that $OPT_\mu \geq \dfrac {OPT} {8\log m}$.
%\end{claim}
%\begin{proof}
%Fix some optimal solution $(O_1,\ldots, O_n)$. For each player $i$ let $a_i$ be the maximizing clause for the bundle $O_i$ in $v_i$. Now, for every player $i$ and every item $j\in O_i$, put item $j$ into bin $x$, where $x$ is a power of $2$, if and only if $2x>a_i(\{j\})\geq x$. Let $M_x$ be the set of items in bin $x$. We claim that there exists bin $\mu$, $\mu \geq \frac {v_{max}} {2m}$, for which it holds that $\Sigma_i \Sigma_{j\in  O_i \cap M_\mu }a_i(\{j\})\geq \frac {\Sigma_i v_i(O_i)} {4\log m}$. To see this, first let $L$ be the set of ``small'' items that are in any of the bins $x$, $x\leq \frac {v_{max}} {4m}$. It holds that $\Sigma_i\Sigma_{j\in O_i \cap L}a_i(\{j\})\leq \Sigma_i\Sigma_{j\in O_i \cap L} \frac{v_{max}}{2m}\leq \frac {v_{max}} 2 \leq \frac {\Sigma_iv_i(O_i)} 2$. Thus, we have that $\Sigma_{i} v_i(O_i \cap \cup_{x\in \mathcal M} M_x) \geq \frac {\Sigma_iv_i(O_i)} 2$. Now observe that the number of bins $x$, $x\geq  \frac {v_{max}} {2m}$ is bounded from above by $2\log m$. Therefore, there exists a bin $\mu$ such that $\Sigma_{i} v_i(O_i \cap M_\mu) \geq \frac {\Sigma_iv_i(O_i)} {4 \log m}$. The proof is completed by observing that $\Sigma_{i} v^{\mu}_i(O_i \cap M_\mu) \geq \frac{1}{2} \Sigma_{i} v_i(O_i \cap M_\mu)$ as the $\mu$-projection cuts the value of each of the item by at most half.
%
%%For each $i$, let $O'_i=O_i\cap M_{\mu}$. It holds that $2 \cdot \sum_i v^{\mu}_i(O'_i) \geq\Sigma_{j\in M_{x}}a_i(\{j\})  \geq \frac {\Sigma_iv_i(O_i)} {4\log m}$. The first transition is due to the fact that the value of every item $j\in O'_i$ in the maximizing clause of $O'_i$ of the projection $v^{ \mu}_i$ is at least half of its value in $a_i$. 
%\end{proof} 
%
%\end{proof}
%
%\begin{lemma}
%If there exists a simultaneous algorithm for $t$-restricted instances that provides an approximation ratio of $\alpha$ where each bidder sends a message of length $l$, then there exists a simultaneous algorithm for binary XOS bidders (with the same $\mu$) that provides an approximation ratio of $O(\alpha\cdot \log m)$ where each bidder sends a message of length $O(l \cdot \log m)$.
%\end{lemma}
%\begin{proof}
%We will show that for every instance of combinatorial auctions with binary XOS bidders there exists some $t$ for which  this instance is $t$-restricted. Given algorithms $A_t$ for $t$-restricted instances we can construct an algorithm for binary XOS valuations as follows: for each $t\in \{1,2,4, \ldots, m\}$ each bidder sends the same message as in $A_t$. Now compute $\log m+1$ allocations, one for each value of $t$, and output the allocation with the highest value.
%
%We now show the existence of one ``good'' $t$ as above. Let $(O_1,\ldots O_n)$ be some optimal solution. Put the players into $\log m$ bins, where player $i$ is in bin $r$ if $2r>|O_i|\geq r$, for $r\in \{1,2,4, \ldots, m\}$. Let $N_r$ be the set of players in bin $r$. Let $t=\arg\max_r\Sigma_{i\in N_r}v_i(O_i)$. For each $i$ let $A_i$ be an arbitrary subset of $O_i$ of size $t$ if $i\in N_t$ and $A_i=\emptyset$ otherwise. We have that $\Sigma_iv_i(A_i) \geq \frac{\Sigma_{i\in N_t}v_i(O_i)}{2}\geq \frac {\Sigma_iv_i(O_i)} {4\log m}$.
%\end{proof}
%}


\prevproof{Theorem}{thm-xos-alg}{
The three claims regarding the approximation ratios are a part of the next lemma which shows that the algorithm achieves the specified approximation ratio.

\begin{lemma}\label{lemma-xos-alg-proof}
Let $(A_1,\ldots, A_n)$ be the allocation that is guaranteed by the $t$-restrictness of the instance. Let $(T_1,\ldots,T_n)$ be the allocation that the algorithm outputs. Then, $\frac{\sum_i v_i(A_i)}{\sum_i v_i(T_i)} \leq \tilde O(m^{1/3})$.
\end{lemma}
\begin{proof}
We first show that every player $i$ reports a large fraction of $A_i$ (but the  items of $A_i$ might be split among different reported bundles).  
\begin{claim}\label{claim-alg-t/2}
For each player $i$, let $\Phi_i=A_i\cap (\cup_{T\in \mathcal S_i}T)$. We have that $|\Phi_i|\geq t/2$.
\end{claim}
\begin{proof}
Suppose that there exists some player $i$ such that $|\Phi_i|<t/2$, and let $S=A_i-(\cup_{T\in\mathcal S_i}T)$. Since $|A_i|= t$, we have that $|S|\geq t/2$. But then the set $\mathcal S_i$ is not maximal, since any subset of the bundle $S$ of size of $t/2$ could have been added to it.
\end{proof}

\begin{corollary}
$\Sigma_iv_i(\Phi_i) \geq  \frac {\Sigma_i v(A_i)} {2}$.
\end{corollary}

We now divide the players into $\log m$ bins so that player $i$ is in bin $r$ if $r>|\mathcal S_i|\geq \frac r 2$. Let the set of players in bin $r$ be $N_r$. Observe that there has to be some bin $l$ with $\Sigma_{i\in N_l}v_i(\Phi_i)\geq \frac {\Sigma_iv_i(\Phi_i)} {\log m}$. Denote its size by $n_l=|N_l|\leq n'$. For the rest of this proof we will only consider the players in $N_l$; this will result of a loss of at most $\log(m)$ in the approximation factor. 

\begin{claim}[$\tilde O(t)$-approximation]\label{claim-approx-t}
$\Sigma_{i\in N_l} v'_i(T_i)\geq \Sigma_i v_i(\Phi_i)/(t \cdot \log(m))$.
\end{claim}
\begin{proof}
We show that there exists an allocation $(B_1,\ldots, B_n)$, $|B_i|\leq 1$ for all $i$, with $\Sigma_iv'_i(B_i)\geq 2\Sigma_iv_i(\Phi_i)/t$. For each player $i\in N_l$, let $B_i$ be the set that contains exactly one item $j_i$ from $\Phi_i$ if $\Phi_i\neq\emptyset$ and $B_i=\emptyset$ otherwise. Notice that the $j_i's$ are distinct, since for every $i\neq i'$ we have that $\Phi_i\cap \Phi_{i'}=\emptyset$. The lemma follows since $v'_i(\{j_i\})=1$.
\end{proof}

\begin{claim}[$\tilde O(l)$-approximation]\label{claim-approx-l}
$\Sigma_{i\in N_l} v'_i(T_i)\geq \Sigma_iv_i(\Phi_i)/( l\cdot \log m)$.
\end{claim}
\begin{proof}
For each player $i\in N_l$, let $B_i \subseteq \Phi_i$ be the bundle of the maximal size such that $v'_i(B_i)=|B_i|$. Note that $|B_i|\geq |\Phi_i|/l$ as by construction $v'_i$ has at most $l$ clauses and by definition each item in $\Phi_i$ is contained in one of the $|\mathcal S_i|$ clauses of $v'_i$. Therefore, $|B_i|\geq |\Phi_i|/l$. Thus we have that $\Sigma_{i\in N_l} v'_i(B_i)\geq \frac {\Sigma_{i\in N_l}v_i(\Phi_i)} {l}$. The claim follows as we already observed that $\Sigma_{i\in N_l}v_i(\Phi_i)\geq \frac {\Sigma_iv_i(\Phi_i)} {\log m}$. 
\end{proof}

\begin{claim}[$\tilde O(n'/l)$-approximation]\label{claim-approx-n/l}
$\Sigma_{i\in N_l} v'_i(T_i)\geq \frac{4n_l}{l} \cdot \frac{\Sigma_{i} v_i(\Phi_i)}{\log(m)}$.
\end{claim}
\begin{proof}
Consider the following experiment. For each player in $N_l$ choose uniformly at random a bundle to compete on among the bundles in the set $\mathcal S_i$ (recall that $\frac{l}{2}  \leq |\mathcal S_i|< l$). Now allocate each item $j$ uniformly at random to one of the players that are competing on bundles that contain that item $j$.

There are $n_l$ players in this experiment, so there are at most $n_l$ potential competitors for each item. Each player has at least $l/2$ disjoint potential bundles to compete on, hence the expected number of competitors on each item is at most $2n_l/l$. So when player $i$ is competing on a bundle, the expected competition on each of the items he competes on is $2n_l/l+1$. Therefore, the expected contribution of each item that player $i$ is competing on is at least $\frac {l} {2n_l}$. The lemma follows by applying linearity of expectation on the (at least) $t/2$ items that are in the bundle that player $i$ is competing on. Therefore we have that  $\Sigma_{i\in N_l} v'_i(T_i)\geq \frac {l} {2n_l} \cdot \frac{t}{2} \cdot {n_l} = \frac{l\cdot t}{4}$. Recall that $\frac{\Sigma_{i} v_i(\Phi_i)}{\log(m)} \leq \Sigma_{i\in N_l} v_i(\Phi_i) \leq t \cdot n_l $. Thus we have that $\frac{l\cdot t}{4} \geq \frac{4n_l}{l} \cdot \frac{\Sigma_{i} v_i(\Phi_i)}{\log(m)}$ as required. 
\end{proof}

Lemma \ref{lemma-xos-alg-proof} now follows by applying Claim \ref{lemma-xos-alg-combined}.
\end{proof} }

%\prevproof{Theorem}{thm-xos-rounds}{
%In the analysis we fix some optimal solution $(O_1,\ldots, O_n)$. We break the proof of the theorem into two lemmas.
%
%\begin{lemma}\label{claim-xos-rounds-ends}
%At the end of the algorithm, either for every player $i$ that did not receive any bundle we have that $U_{k+1,i}=\emptyset$, or the approximation ratio of the algorithm is $O(m^{\frac 1 {k+1}})$.
%\end{lemma}
%\begin{proof}
%Observe the for every player $i$ and round $r$, if $i \in N_r \cap N_{r+1}$ then $|\cup_{S \in \mathcal{S}_{r,i}} S| \geq m^{\frac{1}{k+1}} |\cup_{S \in \mathcal{S}_{r+1,i}} S|$. This is true since if player $i$ was not allocated any items at round $r$ then for every bundle $S \in \mathcal{S}_{r,i}$ that he reported, at least $(1-\frac{1}{m^{\frac{1}{k+1}}})$ of the items were allocated. Thus, $m^{\frac{1}{k+1}} \cdot|U_{r+1,i}| \leq |\cup_{S \in \mathcal{S}_{r,i}} S|$. Recall that by definition we have that $(\cup_{S \in \mathcal{S}_{r+1,i}} S) \subseteq U_{r+1,i}$. Therefore, for every player $i$ that was not allocated anything at round $k$, we have that $|U_{k+1,i}| \leq m^{\frac{1}{k+1}}$. If there exists a player $i$ such that $|U_{k+1,i}| >0$ then it has to be the case that initially $|\cup_{S \in \mathcal{S}_{1,i}} S|\geq m^{\frac k {k+1}}$. This implies that at least $m^{\frac k {k+1}}-m^{\frac{1}{k+1}}$ of the items were allocated and hence the approximation ratio is $O(m^{\frac 1 {k+1}})$ (there are $m$ items, so the value of the optimal solution is at most $m$). In any other case for every player that was not allocated any bundle we have that $U_{k+1,i}=\emptyset$.
%\end{proof}
%
%\begin{lemma}
%Suppose that for every player $i$ that did not receive any bundle we have that $U_{k+1,i}=\emptyset$. The approximation ratio of the algorithm is $O(k\cdot m^{\frac 1 {k+1}})$.
%\end{lemma}
%\begin{proof}
%Suppose that at least $n'/2$ players were allocated non empty bundles. The value of the bundle that each player was allocated is at least $\frac{t}{2k \cdot m^{\frac 1 {k+1}}}$. Thus, in this case the algorithm achieves an $O(k\cdot m^{\frac 1 {k+1}})$-approximation (recall that the value of the optimal solution is $n'\cdot t$). Else, assume that at most $n'/2$ players were allocated some bundle. Consider player $i$ in $N'$ that did not receive any items (there are at least $n'/2$ such players). We will show that for each such player $i$, $|O_i \cap U_{k}| \leq t/4$. In other words, we will show that for every such player $i$, the algorithm allocates at least $\frac {3t} {4}$ of the items that this player receives in the optimal solution. This will prove an approximation ratio of $O(k\cdot m^{\frac 1 {k+1}})$. 
%
%Thus assume towards contradiction that there exists some $i\in N$ that did not receive any items for which $|O_i \cap U_{k}| \geq 3t/4$. In this case by Claim \ref{clm:ind} (below) we have that $|O_i \cap U_{k,i}| \geq \frac{3t}{4}-  k \cdot \frac{t}{2k} = \frac{t}{4}$. In particular this implies that $|U_{k,i}| \geq t/4$. This is a contradiction to the assertion of Lemma \ref{claim-xos-rounds-ends} that $U_{k,i} = \emptyset$ for every player that was not allocated any bundle.
%\end{proof}
%
%\begin{claim} \label{clm:ind}
%For every $i\in N_r\cap N'$, $|O_i \cap U_r| - |O_i \cap (\cup_{S \in \mathcal{S}_{r,i}} S)| \leq r \cdot \frac{t}{2 k}$. 
%\end{claim}
%\begin{proof}
%We prove the claim by induction. For the base case $r=1$, observe that since player $i$ reports a maximal set of bundles of value $\frac{t}{2k}$ at most $\frac{t}{2k}$ items of his optimal bundle may not be reported by him -- otherwise, those items can be bundled together and added to $\mathcal S_{r,i}$, contradicting maximality. We now assume correctness for $r$ and prove for $r+1$. We have that $|O_i \cap U_r| - |O_i \cap (\cup_{S \in \mathcal{S}_{r,i}} S)| \leq r \cdot \frac{t}{2 k}$. Denote the items allocated at round $r$ by $A_r$. We have that $|O_i \cap (U_r \setminus A_r)| - |O_i \cap (\cup_{S \in \mathcal{S}_{r,i}} S) \setminus A_r| \leq r \cdot \frac{t}{2 k}$ since $\cup_{S \in \mathcal{S}_{r,i}} S) \subseteq u_r$. By definition, this implies that $|O_i \cap U_{r+1}| - |O_i \cap u_{r+1,i})| \leq r \cdot \frac{t}{2 k}$. The proof is completed by observing that $|O_i \cap U_{r,i}|-|O_i \cap (\cup_{S \in \mathcal{S}_{r,i}} S)| \leq \frac{t}{2 k}$. Since in every round player $i$ reports a maximal disjoint set of bundles of size $\frac{t}{2 k}$, thus at every round the player can leave out of its reported set at most $\frac{t}{2 k}$ items from the optimal solution (i.e., if the player leaves out more items then he could have reported those items, contradicting maximality).
%\end{proof} }

==> app/xos-app.tex <==
% !TEX root = ..//communism.tex


\section{Proofs from Section \ref{sec-xos-lb}}

%\prevproof{Lemma}{lemma-xos-lb-opt}{
%%\begin{proof}
%Consider allocating each player $i$ the set $T_i$ (an item $j$ that is in multiple $T_i$'s will be allocated to some player $i$ such that $j \in T_i$). The social welfare of this allocation is 
%$|\cup_i T_i|$. We show that with high probability the social welfare is $\Theta(k^4)$. This follows since each $T_i$ is of size $k$ and is practically selected uniformly at random from a set of size $k^4$. Thus, the probability that item $j$ is in $T_i$ is $1/k^3$. Since there are $k^3$ players, an item is in $\cup_i T_i$ with constant probability. Next, since items are chosen independently we can use Chernoff bounds to get that with high probability a constant fraction of all items is in $\cup_i T_i$.
%%\end{proof}
%}

%\prevproof{Lemma}{lemma-set-seeking}{
%Fix a message $m$ and let $A_m(P)$ denote the set $A$ that the seeker returns when his input is $P$ and the keeper sends a message $m$.
%\begin{definition}
%Fix a message $m$ and a set $P$, $|P|=k^2$. A set $S$ is \emph{$(m,P)$-compatible} if $|A_m(P) \cap S| \geq \dfrac{|A_m(P)|}{k^{1-\epsilon}}$.
%\end{definition}
%
%\begin{claim}\label{claim-m-compatible}
%Fix a message $m$ and a set $P$, $|P|=k^2$. The probability that a set $S$ which is chosen uniformly at random from $P$ is $(m,P)$-compatible is at most $e^{-k^\epsilon}$.
%\end{claim}
%\begin{proof}
%We fix a set $A_m(P)=A\subseteq P$ and compute the probability that the intersection of this set with a set $S$ of size $k$ chosen uniformly at random out of $k^2$ items will be greater than $\dfrac{|A|}{k^{1-\epsilon}}$. The probability of each element in $S$ to be in $A \cap S$ is exactly $\dfrac{|A|}{k^2}$. Thus we expect that $|A \cap S| \approx \dfrac{|A|}{k}$. We now use Chernoff bounds to make this precise. We can think of the set $S$ as constructed in the following manner: there are $k$ independent variables, each variable $y_i$ is true with probability $\dfrac{|A|}{k^2}$ and false with probability $1-\dfrac{|A|}{k^2}$. Let $Y=\sum_i y_i$. Let $S$ be constructed by choosing uniformly at random a set of size $Y$ from $A$ and a set of size $k-Y$ from $P\setminus A$. Observe that the distribution of a set constructed this way is identical to choosing $S$ uniformly at random. The expectation of $Y$ is $\dfrac{|A|}{k}$. Now by Chernoff bounds we get that: $\Pr[Y> k^\epsilon \cdot \dfrac{|A|}{k} ] \leq \left (\dfrac{1}{e^{k^\epsilon}}\right )^{\dfrac{|A|}{k}} \leq  \dfrac{1}{e^{k^\epsilon}}$. The last transition holds by the assumption that $|A|\geq k$.
%\end{proof}
%
%\begin{definition} \label{def-f-good}
%Let $F$ be a family of sets of size $k$, $|F|=t=e^{2k^\epsilon}$. We say that a message $m$ is \emph{$F$-good} if $\Pr[|A_m(P)\cap T|\geq \dfrac {|A_m(P)|} {k^{1-\epsilon}}]\geq e^{-\frac 1 2 k^\epsilon}$, where $T$ is chosen uniformly at random from $F$ and $P$, $|P|=k^2$, contains $T$ and $k^2-k$ items chosen uniformly at random from the rest of the items.
%\end{definition}
%
%\begin{claim}
%For every message $m$, the probability that $m$ is $F$-good is at most \[p'=e^{{(-\frac 1 2k^\epsilon)}^{(e^{k^\epsilon)}}}\]where the sets in $F$ are chosen uniformly at random.
%\end{claim}
%\begin{proof}
%Fix a message $m$. Consider $F$ where the sets in $F$ are chosen uniformly at random. We first compute the probability that for a single $T \in F$ we have that $|A_m(P)\cap T|\geq \dfrac {A_m(P)} {k^{1-\epsilon}}$. Observe that every set $T \in F$ in this setting can be thought of as chosen uniformly at random from a fixed set $P$. Thus that probability is the same as the probability that $T$ is $(m,P)$-compatible, which is $e^{-k^\epsilon}$ by Claim \ref{claim-m-compatible}.
%
%Now we would like to compute the probability that $m$ is $F$-good, that is the probability that there are at least $e^{-\frac 1 2 k^\epsilon}\cdot |F| = e^{\frac 3 2 k^\epsilon}$ of the sets $T\in F$ such that  $|A_m(P)\cap T|\geq \dfrac {|A_m(P)|} {k^{1-\epsilon}}$. The expected number of such sets is $e^{-k^\epsilon} \cdot |F|=e^{k^\epsilon}$. By the Chernoff bounds ($\mu=e^{k^\epsilon}$, $\delta=e^{\frac 1 2 k^\epsilon}$) this probability is at most $p'$.
%\end{proof}
%
%We can now finish the proof. Choose $F$ at random. For every $m$ the probability that $m$ is $F$-good is at most $p'$. The message length is $l$, and the total number of messages is therefore at most $2^l$. Thus, by the union bound, the probability that there exists some message $m$ which is $F$-good is at most $2^l\cdot p'\leq 2^{t^\epsilon}  \cdot p' = 2^{e^{k^{\epsilon^\epsilon}}}  \cdot p'< (2e^{(-\frac 1 2k^\epsilon)})^{{(e^{k^\epsilon)}}} <e^{-e^{k^\epsilon}}$, where the transition before the last uses the fact that $\epsilon<1$. Hence, with probability at least $1-e^{-e^{k^\epsilon}}$ every message $m$ is not $F$-good for the randomly chosen $F$. This in turn implies that for a family $F$ and for every $m$ the probability for $P$ and $T$ chosen as in Definition \ref{def-f-good} that $T$ is $(m,P)$-compatible is at most $e^{-\frac 1 2 k^\epsilon}$. Thus, with probability $1-e^{-e^{k^\epsilon}}-e^{-\frac 1 2 k^\epsilon}$ we have that $|A_m(P)\cap T|\leq \dfrac {|A_m(P)|} {k^{1-\epsilon}}$ and thus the approximation ratio is $k^{1-\epsilon}$. Even if with probability $e^{-e^{k^\epsilon}}-e^{-\frac 1 2 k^\epsilon}$ the approximation ratio is $1$, the expected approximation ratio is at most $2k^{1-\epsilon}$. 
%}

%\prevproof{Lemma}{lemma-xos-reduction}{
%In the proof we fix an algorithm for the multi-player combinatorial auction problem and analyze its properties.
%\begin{definition}
%Fix an algorithm for the XOS problem and consider the distribution $D$. We say that player $i$ is \emph{good} if $E[|A_i\cap T_i|]\geq \max \{ \dfrac{|A_i|}{k^{1-\epsilon}}, k^{\epsilon} \}$.
%\end{definition}
%
%\begin{claim}
%If none of the players is good than the expected approximation ratio is at most $m^{\frac 1 4 - \epsilon}$.
%\end{claim}
%\begin{proof}
%To give an upper bound on the expected social welfare we assume that all items in the center are always allocated to players that demand them. We now compute an upper bound on the contribution of the remaining $k^4$ items to the expected social welfare.
%Observe that each player contributes at most $\dfrac{|A_i|}{k^{1-\epsilon}}+ k^{\epsilon}$ to the expected social welfare (of the $k^4$ items). Hence the expected social welfare achieved by the algorithm is at most $\sum_i(\dfrac{|A_i|}{k^{1-\epsilon}}+k^\epsilon) +|C|  = \dfrac{k^4}{k^{1-\epsilon}} + k^3\cdot k^\epsilon +k^3 \leq 3k^{3+\epsilon}$. This implies that the approximation ratio of the algorithm is $k^{1-\epsilon} \leq m^{\frac 1 4 - \epsilon}$.
%\end{proof}
%
%\begin{claim}
%If there exists a good player then there exists an algorithm for the two-player set seeking problem that guarantees an approximation ratio of $k^{1-\epsilon}$ with the same message length.
%\end{claim}
%\begin{proof}
%Let player $i$ be the good player. Recall that $D$ is the distribution for the multi-player combinatorial auction and that $D_2$ is the distribution defined for the set seeking problem. We denote by $E_{D}[\cdot]$ and $E_{D_2}[\cdot]$ expectations taken over the distributions $D$ and $D_2$ respectively. We show that there exists an algorithm for the set seeking problem achieving expected approximation ratio of $k^{1-\epsilon}$ on $D_2$. 
%
%Let the keeper take the role of player $i$ in the multi-player algorithm and the seeker play the roles of the rest of the $n-1$ players. More precisely, the keeper first sends player $i$'s message to the seeker and then the seeker simulates the messages of the remaining players and run the algorithm internally. This simulation is possible by the assumption that in the multi-player algorithm all messages are sent simultaneously. The number of items in the combinatorial auction will be $k^3+k^4$, where the $x$ items of the set seeking problem will correspond to some set $X$ of size $x$ of items in the combinatorial auction. We first show that given that the information of the seeker and keeper is drawn in a correlated way from $D_2$, they have enough information to simulate the correlated distribution $D$. 
%
%The input of the keeper is defined in a straightforward way, where each set in $F$ defines a clause in the XOS valuation. All items in these clauses are subsets of $X$. The seeker constructs the valuations of the other $n-1$ players as follows: the items that are in $X \setminus P$ form the center. Next the seeker chooses uniformly at random for each player $j$ a petal $P_j$ of the $k^4$ items not in the center, a set $T_j \subseteq P_j$ of size $k$ and additional $t-1$ sets of size $k$ from $C\cup P_j$. Observe that the distribution of valuations constructed this way is identical to $D$. The inherent reason for this is that for player $i$ the distribution of $P_i$ and $T_i$ is identical to the distribution of $P$, $T$ and $F$ in $D_2$ as in both cases $P$ and the $t-1$ sets in $F$ (or $P_i$ and $F_i$) are chosen uniformly at random from a set of size $k^3+k^2$ and $T$ (or $T_i$) is chosen uniformly at random from $P$ (or $P_i$). In other words, the distribution $D_2$ on $F,P$ and $T$ is identical to distribution $D$ projected on $F_i,P_i$ and $T_i$.
%
%
%We now observe that since $i$ is a good player we have that $E_D[|A_i\cap T_i|]\geq \max \{ \dfrac{|A_i|}{k^{1-\epsilon}}, k^{\epsilon} \}$. We show that this implies an algorithm achieving expected approximation ratio of $k^{1-\epsilon}$ for the two-player set seeking problem. The algorithm works as follows: we first perform the reduction above, and therefore the distribution we are analyzing is $D$. Now, if player $i$ was assigned a bundle $A_i$ of size at least $k$, the algorithm returns $A=A_i$. Else, the algorithm returns a bundle $A$ that contains $A_i$ and additional $k-|A_i|$ arbitrary items. Thus, we have that $E_D[|A\cap T_i|]\geq \dfrac{|A|}{k^{1-\epsilon}}$, as we made sure that $|A|\geq k$ implying that $\dfrac{|A|}{k^{1-\epsilon}}\geq k^\epsilon$.
%
%We claim that the expected approximation ratio of the algorithm on $D_2$ is $k^{1-\epsilon}$. As the distribution $D_2$ on $F,P$ and $T$ is identical to distribution $D$ projected on $F_i,P_i$ and $T_i$, we have that $E_{D_2}[|A\cap T|]\geq \dfrac{|A|}{k^{1-\epsilon}}$. Thus, $E_{D_2}[\dfrac{|A\cap T|}{|A|}]\geq \dfrac{1}{k^{1-\epsilon}}$. This in turn implies that $\max_{S \in F} \dfrac{|A \cap S|}{|A|} \geq \dfrac{1}{k^{1-\epsilon}}$ and since the optimal solution has a value of $1$ the expected approximation ratio is $k^{1-\epsilon}$.
%\end{proof}
%
%From the last two claims we get that either the algorithm for the combinatorial auction problem does not guarantee a good approximation ratio, or that we have constructed an efficient protocol for the set seeking problem.
%
%}
